Finger Grip Force Estimation from Video using Two Stream Approach

Estimation of a hand grip force is essential for the understanding of force pattern during the execution of assembly or disassembly operations. Human demonstration of a correct way of doing an operation is a powerful source of information which can be used for guided robot teaching. Typically to assess this problem instrumented approach is used, which requires hand or object mounted devices and poses an inconvenience for an operator or limits the scope of addressable objects. The work demonstrates that contact force may be estimated using a noninvasive contactless method with the help of vision system alone. We propose a two-stream approach for video processing, which utilizes both spatial information of each frame and dynamic information of frame change. In this work, image processing and machine learning techniques are used along with dense optical flow for frame change tracking and Kalman filter is used for stream fusion. Our studies show that the proposed method can successfully estimate contact grip force with RMSE < 10% of sensor range (RMSE $\approx 0.2$ N), the performances of each stream and overall method performance are reported. The proposed method has a wide range of applications, including robot teaching through demonstration, haptic force feedback, and validation of human- performed operations.

==> rtos_comparison_tabular.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
RTOS feature & eCos & uc/OS-II & scmRTOS & freeRTOS \\ \hline
Free of charge & +/- & - & + & + \\ \hline
Open-source & + & + & + & + \\ \hline
Required functions support & +++ & ++ & + & ++ \\ \hline
Port for STM & +/- & + & + & + \\ \hline
Small footprint size & ++ & + (5-24KB) & +++ ($\sim 2$ KB) & ++ (5-10KB) \\ \hline
Different architecture support & ++ & +++ & ++ & +++ \\ \hline
Context switching speed & ? & ? & ++ ($1-2 \mu \textrm{s}$) & +++ ($\sim 1 \mu \textrm{s}$) \\ \hline
Number of processes & ? & ++ (250) & + (31) & +++ (limited by RAM) \\ \hline
Documentation quality, availability of examples & + & + & +++ & +++ \\ \hline
\end{tabular}


==> screw_recognition_tabular.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline &
\bf {Train IoU, \%} &
\bf {Validation IoU, \%} &
\bf {Forward time, ms } &
\bf {Screws detected, \%}
%\bf \shortstack{Screws detected,\\controlled conditions, \%}
\\
\hline
\bf SSD &
63.05 &
61.42 &
1450 &
-\\
\hline
\bf UNet &
66.12 &
64.42 &
2700 &
60 \\
\hline
\bf SegNet &
48.39 &
40.66 &
850 &
61\\
\hline
\bf SegNet + HN$^*$ &
67.95 &
66.08 &
850 &
63\\
\hline
\bf \shortstack{SegNet + HN$^*$ + WL$^{**}$} &
68.44 &
66.83 &
850 &
62\\
\hline
\end{tabular}

